Online Extrinsic Calibration based on Per-Sensor Ego-Motion Using Dual Quaternions

In this work, we propose an approach for extrinsic sensor calibration from per-sensor ego-motion estimates. Our problem formulation is based on dual quaternions, enabling two different online capable solving approaches. We provide a certifiable globally optimal and a fast local approach along with a method to verify the globality of the local approach. Additionally, means for integrating previous knowledge, for example, a common ground plane for planar sensor motion, are described. Our algorithms are evaluated on simulated data and on a publicly available dataset containing RGB-D camera images. Further, our online calibration approach is tested on the KITTI odometry dataset, which provides data of a lidar and two stereo camera systems mounted on a vehicle. Our evaluation confirms the short run time, state-of-the-art accuracy, as well as online capability of our approach while retaining the global optimality of the solution at any time.

==> img/kitti_path_07_data.tex <==
\addplot [color=mycolor1, line width=2.0pt, forget plot]
table[row sep=crcr]{%
2.220446e-16	-5.551115e-17\\
0.09154274	0.004596714\\
0.1857373	0.01001116\\
0.2834672	0.01753371\\
0.38731	0.02863192\\
0.5011396	0.04273697\\
0.6279359	0.06000009\\
0.7669396	0.08275693\\
0.9191805	0.1090497\\
1.081913	0.1415335\\
1.251378	0.1816057\\
1.425643	0.2325643\\
1.60414	0.293459\\
1.78864	0.3616512\\
1.979231	0.4366243\\
2.17302	0.5224919\\
2.368741	0.620094\\
2.565689	0.7248452\\
2.758285	0.8394934\\
2.950416	0.9687591\\
3.142085	1.103633\\
3.333105	1.242764\\
3.523028	1.392475\\
3.706267	1.564446\\
3.880703	1.761568\\
4.049498	1.969361\\
4.215884	2.187835\\
4.382391	2.415527\\
4.540774	2.663146\\
4.68768	2.929115\\
4.824434	3.215512\\
4.948178	3.517839\\
5.057271	3.836955\\
5.153468	4.17713\\
5.233794	4.534335\\
5.302451	4.911075\\
5.360943	5.299329\\
5.401694	5.701357\\
5.42129	6.122091\\
5.427674	6.558994\\
5.424017	7.009091\\
5.410697	7.473426\\
5.389282	7.950411\\
5.353644	8.444612\\
5.310729	8.953007\\
5.263869	9.480377\\
5.211227	10.02302\\
5.153075	10.57921\\
5.08836	11.15274\\
5.02588	11.73941\\
4.964841	12.34412\\
4.901812	12.96427\\
4.835681	13.60015\\
4.767225	14.25164\\
4.697363	14.91341\\
4.629999	15.59372\\
4.563302	16.29098\\
4.49463	17.00478\\
4.426532	17.73322\\
4.359249	18.47183\\
4.290984	19.22427\\
4.223122	19.98833\\
4.161929	20.7731\\
4.100217	21.56448\\
4.035961	22.36419\\
3.971019	23.16415\\
3.90897	23.9695\\
3.849052	24.78947\\
3.786079	25.61886\\
3.716343	26.46136\\
3.644752	27.30755\\
3.569541	28.15287\\
3.492898	28.99762\\
3.41846	29.83721\\
3.346046	30.67424\\
3.27199	31.51586\\
3.198821	32.35442\\
3.123626	33.19517\\
3.051261	34.02626\\
2.980358	34.86004\\
2.910621	35.69639\\
2.843137	36.53345\\
2.77507	37.37375\\
2.706985	38.21476\\
2.638855	39.04918\\
2.572257	39.88167\\
2.504806	40.71171\\
2.436154	41.5384\\
2.363072	42.3652\\
2.290205	43.19143\\
2.223683	44.01519\\
2.160908	44.83883\\
2.096619	45.66121\\
2.028253	46.48335\\
1.959122	47.30744\\
1.890493	48.12333\\
1.820295	48.93314\\
1.740695	49.73553\\
1.659366	50.53252\\
1.575304	51.32871\\
1.493752	52.12276\\
1.416807	52.9159\\
1.337479	53.70196\\
1.258994	54.484\\
1.184702	55.26303\\
1.110756	56.03808\\
1.032637	56.81074\\
0.956539	57.5746\\
0.883063	58.33039\\
0.8100074	59.07759\\
0.7359683	59.8104\\
0.6623665	60.53658\\
0.5919478	61.24548\\
0.5237598	61.94033\\
0.4617179	62.62022\\
0.4088407	63.28551\\
0.3622951	63.93546\\
0.3201877	64.57047\\
0.2859581	65.18991\\
0.2627668	65.79136\\
0.2555668	66.37563\\
0.2646196	66.93703\\
0.2941699	67.47673\\
0.3455598	67.99052\\
0.4164808	68.48214\\
0.5048813	68.95412\\
0.6110892	69.40376\\
0.7419667	69.84846\\
0.8955753	70.27047\\
1.080744	70.68171\\
1.285746	71.06861\\
1.51356	71.45144\\
1.753829	71.81419\\
2.013647	72.17075\\
2.296944	72.50742\\
2.601772	72.81071\\
2.908665	73.10855\\
3.220823	73.38524\\
3.554385	73.65932\\
3.91127	73.91333\\
4.300551	74.16588\\
4.71851	74.40171\\
5.155827	74.61515\\
5.623155	74.8256\\
6.110247	75.01816\\
6.618096	75.20557\\
7.151976	75.37989\\
7.706095	75.5393\\
8.281091	75.69196\\
8.874404	75.83698\\
9.486418	75.98069\\
10.1122	76.12225\\
10.75522	76.25804\\
11.41499	76.37903\\
12.0915	76.49294\\
12.78422	76.60203\\
13.49407	76.70271\\
14.2125	76.79658\\
14.94545	76.88462\\
15.68785	76.96463\\
16.44684	77.04091\\
17.21856	77.11873\\
17.99359	77.19881\\
18.76754	77.27201\\
19.53401	77.33723\\
20.30151	77.40244\\
21.07246	77.46374\\
21.84296	77.52113\\
22.61434	77.5734\\
23.37766	77.6221\\
24.13827	77.67675\\
24.89811	77.7342\\
25.65478	77.78961\\
26.42191	77.84614\\
27.18067	77.90878\\
27.93923	77.96897\\
28.692	78.02007\\
29.44067	78.06469\\
30.19277	78.1097\\
30.94569	78.15548\\
31.7013	78.1981\\
32.46413	78.24233\\
33.23079	78.29498\\
34.00093	78.34624\\
34.77685	78.39928\\
35.56152	78.44974\\
36.34754	78.50718\\
37.14347	78.57152\\
37.93752	78.63617\\
38.73523	78.7004\\
39.54602	78.7627\\
40.36454	78.82862\\
41.19468	78.89593\\
42.03064	78.95989\\
42.87429	79.02897\\
43.72474	79.10034\\
44.57894	79.1713\\
45.43863	79.24668\\
46.2992	79.31863\\
47.16296	79.38492\\
48.03166	79.44527\\
48.90207	79.50861\\
49.77895	79.57376\\
50.6563	79.63392\\
51.52945	79.69742\\
52.39664	79.76468\\
53.2548	79.83358\\
54.1135	79.90039\\
54.96562	79.96964\\
55.81906	80.03259\\
56.67063	80.09273\\
57.52689	80.15558\\
58.37775	80.22244\\
59.2131	80.28086\\
60.04264	80.33871\\
60.87223	80.40305\\
61.69567	80.47401\\
62.51365	80.54972\\
63.32787	80.62089\\
64.13629	80.69604\\
64.94508	80.7781\\
65.75279	80.85967\\
66.55929	80.94518\\
67.3635	81.03408\\
68.15999	81.12341\\
68.9488	81.21916\\
69.73955	81.31685\\
70.5203	81.42164\\
71.29191	81.54226\\
72.05943	81.66368\\
72.82193	81.78344\\
73.58474	81.91089\\
74.34335	82.0491\\
75.10124	82.18657\\
75.85198	82.32699\\
76.5947	82.46709\\
77.33161	82.61416\\
78.06923	82.76564\\
78.80777	82.93034\\
79.54411	83.10119\\
80.28097	83.28409\\
81.0106	83.46726\\
81.72568	83.6579\\
82.4307	83.85643\\
83.14038	84.05742\\
83.86239	84.26582\\
84.58416	84.49278\\
85.30299	84.72751\\
86.01174	84.96507\\
86.71556	85.2123\\
87.41701	85.46879\\
88.11804	85.72668\\
88.82079	85.99632\\
89.52111	86.28029\\
90.21553	86.56905\\
90.91809	86.86039\\
91.62194	87.15878\\
92.3185	87.47632\\
93.00351	87.8025\\
93.68698	88.11795\\
94.37577	88.42784\\
95.06817	88.74901\\
95.76606	89.08452\\
96.46571	89.41637\\
97.16351	89.74796\\
97.84976	90.08495\\
98.53474	90.42665\\
99.21955	90.77493\\
99.9095	91.13104\\
100.5948	91.48703\\
101.2774	91.84\\
101.9541	92.19617\\
102.6273	92.55294\\
103.2961	92.91478\\
103.9601	93.28321\\
104.6187	93.65046\\
105.2674	94.01507\\
105.9103	94.38211\\
106.5472	94.74824\\
107.1878	95.12335\\
107.8233	95.49621\\
108.4529	95.86451\\
109.0677	96.2232\\
109.6683	96.57402\\
110.2481	96.92077\\
110.8135	97.26338\\
111.3654	97.60083\\
111.9025	97.92433\\
112.4233	98.24175\\
112.9252	98.55027\\
113.4056	98.84348\\
113.8657	99.12485\\
114.3023	99.39682\\
114.7173	99.66423\\
115.1137	99.91884\\
115.4941	100.1623\\
115.8608	100.3993\\
116.2046	100.6332\\
116.5286	100.8652\\
116.8348	101.0904\\
117.1266	101.3056\\
117.4011	101.506\\
117.6574	101.6929\\
117.8992	101.8739\\
118.122	102.0513\\
118.3256	102.2292\\
118.5086	102.4053\\
118.6815	102.576\\
118.838	102.742\\
118.9816	102.9018\\
119.116	103.0684\\
119.2422	103.245\\
119.3668	103.4183\\
119.4976	103.5947\\
119.6238	103.7731\\
119.7348	103.9548\\
119.8384	104.1481\\
119.9342	104.3385\\
120.0291	104.5336\\
120.1137	104.733\\
120.1854	104.9312\\
120.2566	105.1362\\
120.3283	105.3437\\
120.3886	105.5582\\
120.452	105.8016\\
120.5003	106.0565\\
120.5536	106.3408\\
120.5994	106.6408\\
120.6206	106.946\\
120.6402	107.2795\\
120.6434	107.6301\\
120.6163	107.9733\\
120.5908	108.3468\\
120.5308	108.7113\\
120.4648	109.1034\\
120.3764	109.5039\\
120.2526	109.8936\\
120.1212	110.3105\\
119.9688	110.7358\\
119.7761	111.1598\\
119.5688	111.6037\\
119.3248	112.0419\\
119.0622	112.4967\\
118.7686	112.9599\\
118.447	113.4215\\
118.1067	113.8987\\
117.7492	114.379\\
117.3755	114.8756\\
116.9889	115.3845\\
116.5875	115.9072\\
116.1705	116.4394\\
115.7373	116.978\\
115.2919	117.5268\\
114.8352	118.0864\\
114.3662	118.6599\\
113.8874	119.2396\\
113.3947	119.8351\\
112.8933	120.4389\\
112.3812	121.0569\\
111.8577	121.687\\
111.3222	122.3282\\
110.7728	122.9704\\
110.2135	123.6258\\
109.6502	124.2849\\
109.0798	124.9562\\
108.5006	125.6369\\
107.9136	126.332\\
107.3179	127.0372\\
106.7132	127.7453\\
106.1014	128.4619\\
105.4824	129.186\\
104.8515	129.9193\\
104.2149	130.6623\\
103.5744	131.4132\\
102.9386	132.1648\\
102.3035	132.9234\\
101.6681	133.6799\\
101.0301	134.4357\\
100.3904	135.1892\\
99.75107	135.9465\\
99.10851	136.7105\\
98.46944	137.4685\\
97.82785	138.2274\\
97.18269	138.9901\\
96.54609	139.748\\
95.90422	140.5111\\
95.26259	141.2656\\
94.62044	142.0208\\
93.97889	142.7704\\
93.337	143.5294\\
92.69067	144.2862\\
92.04892	145.0409\\
91.41052	145.794\\
90.77404	146.5475\\
90.13928	147.3072\\
89.50321	148.0704\\
88.87146	148.8333\\
88.23696	149.6005\\
87.60683	150.3591\\
86.97809	151.1134\\
86.34989	151.8671\\
85.71894	152.6218\\
85.08539	153.379\\
84.45676	154.1322\\
83.83215	154.8823\\
83.20615	155.6292\\
82.57906	156.3743\\
81.95146	157.119\\
81.32671	157.8614\\
80.70349	158.6032\\
80.08383	159.3358\\
79.46455	160.0585\\
78.84428	160.7804\\
78.22487	161.5\\
77.60858	162.2213\\
76.99411	162.9402\\
76.38223	163.6585\\
75.77428	164.3767\\
75.17018	165.093\\
74.56637	165.8081\\
73.96713	166.5248\\
73.3721	167.2418\\
72.77838	167.9552\\
72.19108	168.6684\\
71.61267	169.3812\\
71.03558	170.0844\\
70.468	170.7831\\
69.9057	171.4722\\
69.35261	172.1588\\
68.80749	172.8299\\
68.26999	173.4939\\
67.73915	174.1451\\
67.21605	174.7856\\
66.69815	175.4193\\
66.18835	176.0447\\
65.6842	176.6638\\
65.18539	177.2745\\
64.68934	177.8683\\
64.19739	178.4448\\
63.71223	179.0078\\
63.24071	179.5612\\
62.76519	180.1003\\
62.31141	180.6249\\
61.86056	181.1416\\
61.41959	181.6486\\
60.98005	182.1422\\
60.5453	182.6223\\
60.11032	183.0885\\
59.67252	183.5369\\
59.2357	183.9747\\
58.80121	184.4045\\
58.36066	184.8122\\
57.91203	185.1982\\
57.45834	185.5495\\
57.00033	185.8798\\
56.53757	186.1871\\
56.06608	186.455\\
55.59683	186.7152\\
55.12564	186.9445\\
54.64759	187.1206\\
54.17085	187.2835\\
53.69416	187.4227\\
53.21309	187.5256\\
52.7371	187.6307\\
52.25276	187.6915\\
51.77232	187.7485\\
51.29098	187.7723\\
50.80341	187.7414\\
50.33042	187.7165\\
49.86716	187.6828\\
49.40375	187.6045\\
48.95472	187.5198\\
48.50872	187.3856\\
48.08322	187.2454\\
47.66758	187.0919\\
47.2498	186.905\\
46.84089	186.7142\\
46.43056	186.4782\\
46.02498	186.2433\\
45.62057	185.9999\\
45.21752	185.7437\\
44.82494	185.4762\\
44.4335	185.1904\\
44.04415	184.8981\\
43.65148	184.5971\\
43.25715	184.2874\\
42.85899	183.9689\\
42.45635	183.6434\\
42.04606	183.3133\\
41.62858	182.9728\\
41.20434	182.6247\\
40.7774	182.2608\\
40.34468	181.8872\\
39.89489	181.5012\\
39.43245	181.1166\\
38.95179	180.7267\\
38.46147	180.3265\\
37.96509	179.9121\\
37.45911	179.4927\\
36.93739	179.0635\\
36.39418	178.6239\\
35.84918	178.1621\\
35.29616	177.6842\\
34.72689	177.1997\\
34.1427	176.7106\\
33.53889	176.2079\\
32.92207	175.6955\\
32.29666	175.1718\\
31.66497	174.6388\\
31.02204	174.1052\\
30.36327	173.559\\
29.69599	173.0021\\
29.02358	172.4382\\
28.34675	171.867\\
27.6606	171.2881\\
26.96332	170.7093\\
26.25927	170.1234\\
25.54622	169.5314\\
24.82358	168.9342\\
24.09784	168.3371\\
23.3687	167.7434\\
22.6392	167.1591\\
21.90866	166.5815\\
21.17959	166.0001\\
20.44842	165.4129\\
19.71467	164.8351\\
18.99252	164.2567\\
18.28024	163.6778\\
17.57387	163.1045\\
16.8568	162.5251\\
16.14389	161.9505\\
15.42915	161.3773\\
14.71206	160.8026\\
14.01383	160.2415\\
13.30347	159.6822\\
12.59096	159.1338\\
11.87586	158.6027\\
11.15361	158.088\\
10.42311	157.5933\\
9.685989	157.1079\\
8.940913	156.6525\\
8.187478	156.2137\\
7.41973	155.8113\\
6.640524	155.4337\\
5.854252	155.0736\\
5.066725	154.7551\\
4.275819	154.4511\\
3.475256	154.1799\\
2.660279	153.9186\\
1.836084	153.6909\\
1.004297	153.4863\\
0.1642828	153.2952\\
-0.6849197	153.1167\\
-1.551019	152.9463\\
-2.422346	152.7936\\
-3.301845	152.6592\\
-4.18441	152.5347\\
-5.081774	152.4224\\
-6.003442	152.3238\\
-6.932667	152.2301\\
-7.875658	152.1344\\
-8.818435	152.0349\\
-9.767273	151.9309\\
-10.72343	151.8222\\
-11.69649	151.7054\\
-12.68601	151.5906\\
-13.68436	151.4796\\
-14.68941	151.3681\\
-15.70974	151.2539\\
-16.72996	151.1385\\
-17.76061	151.0183\\
-18.79445	150.8986\\
-19.83629	150.7787\\
-20.88457	150.6584\\
-21.93524	150.5418\\
-22.98777	150.4287\\
-24.03963	150.3173\\
-25.09394	150.21\\
-26.14805	150.1008\\
-27.19872	149.9955\\
-28.24318	149.8915\\
-29.28484	149.7898\\
-30.32621	149.6882\\
-31.3652	149.5881\\
-32.40607	149.4892\\
-33.4488	149.3925\\
-34.47237	149.3004\\
-35.50025	149.2116\\
-36.5257	149.1247\\
-37.54989	149.0389\\
-38.57065	148.9571\\
-39.58889	148.8814\\
-40.60275	148.8101\\
-41.61181	148.7352\\
-42.62144	148.6636\\
-43.62164	148.5927\\
-44.62545	148.5176\\
-45.62217	148.4441\\
-46.61393	148.3689\\
-47.60259	148.296\\
-48.59075	148.2258\\
-49.57611	148.1556\\
-50.55843	148.0851\\
-51.53844	148.0135\\
-52.51178	147.9424\\
-53.47973	147.87\\
-54.44853	147.7977\\
-55.41352	147.7243\\
-56.37284	147.6532\\
-57.3302	147.5797\\
-58.2811	147.5001\\
-59.22935	147.4207\\
-60.17164	147.3415\\
-61.10803	147.2599\\
-62.03744	147.1781\\
-62.95647	147.0991\\
-63.86909	147.0218\\
-64.76162	146.9462\\
-65.64189	146.8736\\
-66.50732	146.8046\\
-67.35784	146.7409\\
-68.18896	146.6842\\
-68.99922	146.637\\
-69.78685	146.6018\\
-70.55095	146.575\\
-71.28944	146.5515\\
-72.00342	146.5298\\
-72.68937	146.5152\\
-73.3485	146.5063\\
-73.98191	146.499\\
-74.5886	146.496\\
-75.16771	146.4997\\
-75.72426	146.5087\\
-76.24921	146.5201\\
-76.74501	146.531\\
-77.20836	146.5458\\
-77.64447	146.5624\\
-78.04556	146.5828\\
-78.41532	146.5982\\
-78.7529	146.6147\\
-79.0606	146.6267\\
-79.32694	146.6358\\
-79.57193	146.6444\\
-79.79717	146.6502\\
-79.99877	146.6574\\
-80.19576	146.6613\\
-80.38467	146.6636\\
-80.56988	146.6635\\
-80.74617	146.6558\\
-80.91148	146.6452\\
-81.06159	146.6315\\
-81.20217	146.6264\\
-81.3349	146.6236\\
-81.46093	146.6172\\
-81.58005	146.6064\\
-81.69181	146.591\\
-81.79611	146.5743\\
-81.88799	146.5544\\
-81.96407	146.5371\\
-82.02535	146.5218\\
-82.07268	146.5098\\
-82.10813	146.4988\\
-82.13307	146.4897\\
-82.1479	146.4813\\
-82.15466	146.4749\\
-82.15162	146.47\\
-82.14449	146.4675\\
-82.14289	146.4666\\
-82.14598	146.4691\\
-82.14846	146.4743\\
-82.14814	146.4784\\
-82.14689	146.4809\\
-82.14592	146.4837\\
-82.1443	146.4853\\
-82.14339	146.486\\
-82.14478	146.4874\\
-82.14651	146.4896\\
-82.14732	146.4903\\
-82.15098	146.4929\\
-82.15255	146.4935\\
-82.1546	146.495\\
-82.15536	146.4952\\
-82.15662	146.4961\\
-82.15612	146.4944\\
-82.15657	146.4943\\
-82.15523	146.4929\\
-82.15185	146.4903\\
-82.14843	146.4878\\
-82.14544	146.4858\\
-82.14302	146.4866\\
-82.14091	146.4873\\
-82.13842	146.4876\\
-82.13635	146.4871\\
-82.13505	146.4865\\
-82.13362	146.486\\
-82.13326	146.4879\\
-82.13252	146.4881\\
-82.13297	146.4887\\
-82.13315	146.4887\\
-82.13346	146.489\\
-82.13324	146.4885\\
-82.13358	146.4862\\
-82.13348	146.4847\\
-82.13363	146.485\\
-82.13382	146.4854\\
-82.13351	146.4849\\
-82.13339	146.4851\\
-82.13304	146.4851\\
-82.13367	146.4801\\
-82.13276	146.4764\\
-82.13226	146.4733\\
-82.13189	146.4721\\
-82.13281	146.4755\\
-82.13308	146.4771\\
-82.13322	146.4775\\
-82.13318	146.4765\\
-82.14996	146.506\\
-82.16201	146.525\\
-82.17605	146.5414\\
-82.19557	146.5569\\
-82.2173	146.5659\\
-82.24565	146.5794\\
-82.27544	146.5858\\
-82.31013	146.5906\\
-82.34431	146.5878\\
-82.38439	146.5882\\
-82.42617	146.5818\\
-82.47354	146.578\\
-82.52259	146.5675\\
-82.57422	146.5518\\
-82.63234	146.5331\\
-82.69805	146.5075\\
-82.77848	146.4759\\
-82.88031	146.4452\\
-82.98778	146.3964\\
-83.11671	146.3513\\
-83.25839	146.2958\\
-83.41005	146.2309\\
-83.57444	146.1563\\
-83.74303	146.0701\\
-83.92098	145.9804\\
-84.10616	145.8795\\
-84.29131	145.7599\\
-84.48453	145.6332\\
-84.6826	145.4913\\
-84.88083	145.3153\\
-85.09753	145.1255\\
-85.31851	144.8957\\
-85.56492	144.6601\\
-85.81942	144.3964\\
-86.06536	144.0775\\
-86.32723	143.7422\\
-86.59141	143.3707\\
-86.84062	142.9474\\
-87.08803	142.5033\\
-87.31564	142.01\\
-87.54335	141.5092\\
-87.7514	140.9762\\
-87.92431	140.3921\\
-88.08758	139.7985\\
-88.21988	139.1586\\
-88.33879	138.5086\\
-88.43333	137.8281\\
-88.50147	137.1128\\
-88.56031	136.3792\\
-88.60753	135.6148\\
-88.64646	134.8254\\
-88.67609	134.0129\\
-88.69656	133.1801\\
-88.70556	132.3277\\
-88.70109	131.4527\\
-88.68049	130.552\\
-88.64953	129.6312\\
-88.61212	128.6888\\
-88.57569	127.7239\\
-88.54051	126.7352\\
-88.50489	125.721\\
-88.46433	124.6835\\
-88.4197	123.6288\\
-88.36834	122.5531\\
-88.29428	121.4602\\
-88.21078	120.3502\\
-88.13057	119.2271\\
-88.04055	118.0866\\
-87.94868	116.9301\\
-87.84858	115.7614\\
-87.74507	114.5794\\
-87.63924	113.3837\\
-87.53924	112.1817\\
-87.43868	110.9751\\
-87.34289	109.7745\\
-87.24708	108.5794\\
-87.14676	107.3857\\
-87.04988	106.1976\\
-86.95296	105.0099\\
-86.85966	103.8211\\
-86.76401	102.6322\\
-86.67222	101.4446\\
-86.572	100.2617\\
-86.48067	99.08436\\
-86.38626	97.91011\\
-86.29387	96.73614\\
-86.20143	95.56279\\
-86.11023	94.3923\\
-86.01752	93.22888\\
-85.93007	92.07077\\
-85.8444	90.91482\\
-85.7575	89.76083\\
-85.67406	88.60756\\
-85.59118	87.45822\\
-85.5113	86.31428\\
-85.4316	85.17639\\
-85.35257	84.04212\\
-85.26665	82.90481\\
-85.17822	81.77442\\
-85.08247	80.64658\\
-84.98283	79.52584\\
-84.88244	78.40969\\
-84.78461	77.28896\\
-84.68498	76.17485\\
-84.58436	75.06363\\
-84.48155	73.95599\\
-84.37548	72.84964\\
-84.26751	71.74856\\
-84.1597	70.65049\\
-84.05165	69.5564\\
-83.94657	68.4631\\
-83.84452	67.36871\\
-83.74424	66.26978\\
-83.64855	65.17361\\
-83.55385	64.07225\\
-83.46386	62.98846\\
-83.37192	61.89385\\
-83.27983	60.80165\\
-83.19229	59.72532\\
-83.10582	58.65323\\
-83.02288	57.58891\\
-82.92872	56.51193\\
-82.84557	55.43924\\
-82.75948	54.36293\\
-82.67777	53.28795\\
-82.59449	52.21491\\
-82.50983	51.15105\\
-82.42382	50.10238\\
-82.33696	49.05334\\
-82.25022	48.00472\\
-82.16174	46.96133\\
-82.07717	45.91385\\
-81.99356	44.85398\\
-81.91307	43.795\\
-81.836	42.72975\\
-81.75523	41.66873\\
-81.66958	40.60585\\
-81.5933	39.55165\\
-81.51302	38.49644\\
-81.4292	37.44699\\
-81.34352	36.39931\\
-81.26015	35.35893\\
-81.17846	34.32413\\
-81.09833	33.29069\\
-81.01888	32.26565\\
-80.93893	31.23423\\
-80.86334	30.20542\\
-80.79003	29.18198\\
-80.7195	28.16485\\
-80.65087	27.15493\\
-80.5796	26.14248\\
-80.51287	25.13087\\
-80.44513	24.12616\\
-80.38011	23.12314\\
-80.31382	22.12814\\
-80.2473	21.13624\\
-80.18102	20.15914\\
-80.11803	19.20344\\
-80.05605	18.26545\\
-79.99311	17.34296\\
-79.92964	16.43997\\
-79.86631	15.55805\\
-79.79755	14.70187\\
-79.73095	13.86242\\
-79.65774	13.04799\\
-79.58095	12.25209\\
-79.50525	11.471\\
-79.42836	10.71407\\
-79.34685	9.978597\\
-79.25871	9.267307\\
-79.15904	8.577034\\
-79.05159	7.915426\\
-78.94049	7.272311\\
-78.82344	6.660991\\
-78.69639	6.068827\\
-78.54955	5.472914\\
-78.4073	4.940333\\
-78.24856	4.382647\\
-78.08627	3.86783\\
-77.90275	3.358995\\
-77.71129	2.864838\\
-77.50396	2.385605\\
-77.28713	1.921735\\
-77.05448	1.46975\\
-76.80012	1.027851\\
-76.53314	0.6036779\\
-76.23884	0.2051226\\
-75.91192	-0.166806\\
-75.58157	-0.5205388\\
-75.24181	-0.8592366\\
-74.88301	-1.18203\\
-74.50932	-1.473046\\
-74.11079	-1.733786\\
-73.70973	-1.977241\\
-73.29908	-2.211269\\
-72.8688	-2.4317\\
-72.43254	-2.625592\\
-71.96837	-2.77869\\
-71.5118	-2.915642\\
-71.05343	-3.046312\\
-70.57958	-3.160868\\
-70.1026	-3.257933\\
-69.61007	-3.33279\\
-69.11648	-3.394982\\
-68.61143	-3.452999\\
-68.09683	-3.505748\\
-67.57573	-3.551082\\
-67.04625	-3.59156\\
-66.5056	-3.623078\\
-65.95034	-3.647772\\
-65.37705	-3.663801\\
-64.79002	-3.673887\\
-64.18504	-3.677308\\
-63.56337	-3.675967\\
-62.92543	-3.664022\\
-62.27133	-3.643049\\
-61.60236	-3.617203\\
-60.9157	-3.591227\\
-60.2096	-3.556391\\
-59.49348	-3.520319\\
-58.76038	-3.485568\\
-58.01266	-3.451301\\
-57.2552	-3.415287\\
-56.49375	-3.375737\\
-55.72964	-3.332427\\
-54.96514	-3.288581\\
-54.20352	-3.243097\\
-53.43799	-3.192353\\
-52.67327	-3.132861\\
-51.90721	-3.069795\\
-51.14242	-3.005492\\
-50.37643	-2.937896\\
-49.61228	-2.871709\\
-48.84616	-2.80322\\
-48.0822	-2.741985\\
-47.31871	-2.690256\\
-46.5559	-2.632847\\
-45.79733	-2.573747\\
-45.03968	-2.514617\\
-44.28628	-2.455917\\
-43.53558	-2.395278\\
-42.78704	-2.336487\\
-42.0436	-2.281395\\
-41.30397	-2.229024\\
-40.57423	-2.176053\\
-39.85331	-2.128161\\
-39.14184	-2.080478\\
-38.44127	-2.023801\\
-37.75378	-1.97541\\
-37.0788	-1.93323\\
-36.41471	-1.89552\\
-35.75756	-1.851613\\
-35.10587	-1.807991\\
-34.45818	-1.766675\\
-33.81378	-1.727417\\
-33.17691	-1.687773\\
-32.54447	-1.645582\\
-31.91722	-1.602843\\
-31.29334	-1.561553\\
-30.67447	-1.524724\\
-30.05921	-1.488055\\
-29.44928	-1.45003\\
-28.84028	-1.412389\\
-28.2346	-1.378315\\
-27.63061	-1.340783\\
-27.0287	-1.305986\\
-26.43074	-1.267692\\
-25.83408	-1.229249\\
-25.23953	-1.191105\\
-24.6469	-1.152074\\
-24.06042	-1.111448\\
-23.47692	-1.067365\\
-22.89845	-1.022814\\
-22.3266	-0.9777518\\
-21.76546	-0.9345741\\
-21.21267	-0.8867823\\
-20.67046	-0.8446471\\
-20.14023	-0.8029049\\
-19.61995	-0.7667103\\
-19.1116	-0.7322119\\
-18.61591	-0.6995025\\
-18.132	-0.6673674\\
-17.65726	-0.6355362\\
-17.19632	-0.6017668\\
};

==> img/online_calib_plot_data/rotation_error_data.tex <==

\addplot [color=mycolor2, line width=1pt]
table[row sep=crcr]{%
1	1.77657014337944\\
2	1.12729116362696\\
3	0.897429323718353\\
4	0.777468499653946\\
5	0.776479072908901\\
6	0.889104476539717\\
7	0.676093026974873\\
8	0.536902986931111\\
9	0.588508973800856\\
10	0.508439393020345\\
11	0.422537951269207\\
12	0.403272447052595\\
13	0.364648822050014\\
14	0.370274371900107\\
15	0.339488220878321\\
16	0.337908698952703\\
17	0.363602826309264\\
18	0.336091181204643\\
19	0.345987002168622\\
20	0.344870620529719\\
21	0.348176666754511\\
22	0.334769134012769\\
23	0.327868487566992\\
24	0.341485883159174\\
25	0.335834350931278\\
26	0.327956368681638\\
27	0.324451457374587\\
28	0.321791516744636\\
29	0.322305019261032\\
30	0.322599189678768\\
31	0.325295884927587\\
32	0.323807241467056\\
33	0.326822599453833\\
34	0.325330791463601\\
35	0.323652806289258\\
36	0.324775875154094\\
37	0.328454357292314\\
38	0.326261871542637\\
39	0.33215926218591\\
40	0.33137227659884\\
41	0.338484978846479\\
42	0.353835693573959\\
43	0.328008187311376\\
44	0.364907816935478\\
45	0.370397601632855\\
46	0.36867724751084\\
47	0.365675739621037\\
48	0.327359728077795\\
49	0.3191009678954\\
50	0.318713040599819\\
51	0.318762973746712\\
52	0.31933715349842\\
53	0.319072970579758\\
54	0.318545729199575\\
55	0.318393303922462\\
56	0.318539423077369\\
57	0.319025679771701\\
58	0.320146670036835\\
59	0.319844647193433\\
60	0.318806212057252\\
61	0.318888488423355\\
62	0.319399963836777\\
63	0.318944710142973\\
64	0.320249926356657\\
65	0.318925998615002\\
66	0.319531894758463\\
67	0.320422655636234\\
68	0.32014178948253\\
69	0.320673457927756\\
70	0.320558172573744\\
71	0.318867174239898\\
72	0.319255039975477\\
73	0.31971748831453\\
74	0.31839419543681\\
75	0.319245491229209\\
76	0.318793365759568\\
77	0.319962634170103\\
78	0.320401531509128\\
79	0.320101894943626\\
80	0.319818462944397\\
81	0.320199212585797\\
82	0.319214170178515\\
83	0.319146127377864\\
84	0.319902858690426\\
85	0.319731149439518\\
86	0.319295501077066\\
87	0.319364235144261\\
88	0.32010102075702\\
89	0.319455245392921\\
90	0.319753355507372\\
91	0.319968572657742\\
92	0.319868204230799\\
93	0.320234774173804\\
94	0.320141432962118\\
95	0.319827540134823\\
96	0.319990086495612\\
97	0.320421268520146\\
98	0.320065192518249\\
99	0.320074434726742\\
100	0.319933503653961\\
101	0.319929936332787\\
102	0.319657952427413\\
103	0.319960569197875\\
104	0.320066038492059\\
105	0.319912897137899\\
106	0.319892178931342\\
107	0.319677069492538\\
108	0.320074091392838\\
109	0.319920067027209\\
110	0.319801260317332\\
111	0.320639245004416\\
112	0.32123229850809\\
113	0.322178383596176\\
114	0.321947657863422\\
115	0.322357573714403\\
116	0.323098777810898\\
117	0.323467636230507\\
118	0.323705085115027\\
119	0.324107147926438\\
120	0.324191118295728\\
121	0.323993593207974\\
122	0.324146280481132\\
123	0.32409616061279\\
124	0.324077019452626\\
125	0.324039727930277\\
126	0.324024250977878\\
127	0.324028131548729\\
128	0.324019399934457\\
129	0.324061842247393\\
130	0.324135315486539\\
131	0.324146669577527\\
132	0.324171016206944\\
133	0.324158216111957\\
134	0.324179942936176\\
135	0.324190770302181\\
136	0.324178088053098\\
137	0.324162857091691\\
138	0.324153690215183\\
139	0.324131771294641\\
140	0.324118479309042\\
141	0.32404841504288\\
142	0.324035949160225\\
143	0.32402607851444\\
144	0.323954017054189\\
145	0.323925300352172\\
146	0.324213285690206\\
147	0.324209597408691\\
148	0.324440582035812\\
149	0.323999588977527\\
150	0.324214050600536\\
};

==> img/online_calib_plot_data/time_data.tex <==
\addplot [color=mycolor1, forget plot, line width=1pt]
    table[row sep=crcr]{%
1	0.0864120000000002\\
2	0.0446810000000016\\
3	0.0434900000000003\\
4	0.0447699999999995\\
5	0.0461269999999986\\
6	0.0571570000000007\\
7	0.0426840000000002\\
8	0.0438670000000017\\
9	0.0443660000000005\\
10	0.0435900000000004\\
11	0.0412470000000009\\
12	0.048082000000001\\
13	0.0475510000000003\\
14	0.0503830000000007\\
15	0.0503170000000049\\
16	0.0536539999999988\\
17	0.0509769999999998\\
18	0.0568540000000024\\
19	0.0600399999999999\\
20	0.0521900000000004\\
21	0.0537599999999963\\
22	0.0580680000000025\\
23	0.0570219999999963\\
24	0.0486739999999965\\
25	0.0513600000000007\\
26	0.0523240000000025\\
27	0.0589539999999968\\
28	0.0529919999999944\\
29	0.0499189999999992\\
30	0.051287000000002\\
31	0.0498549999999955\\
32	0.0486749999999968\\
33	0.0501799999999996\\
34	0.0486530000000021\\
35	0.0494180000000039\\
36	0.0504399999999999\\
37	0.0498780000000053\\
38	0.0496010000000023\\
39	0.0522649999999944\\
40	0.0514270000000042\\
41	0.0493030000000022\\
42	0.045465999999998\\
43	0.0540409999999922\\
44	0.0484169999999989\\
45	0.0509649999999968\\
46	0.0486560000000009\\
47	0.047325999999998\\
48	0.0487930000000059\\
49	0.004557\\
50	0.005019\\
51	0.003908\\
52	0.004216\\
53	0.004624\\
54	0.004044\\
55	0.004032\\
56	0.004176\\
57	0.003931\\
58	0.004137\\
59	0.005567\\
60	0.004137\\
61	0.00427\\
62	0.003779\\
63	0.00396\\
64	0.003878\\
65	0.004382\\
66	0.004204\\
67	0.004382\\
68	0.003949\\
69	0.003721\\
70	0.003763\\
71	0.004174\\
72	0.004053\\
73	0.003929\\
74	0.003738\\
75	0.00269\\
76	0.003902\\
77	0.003967\\
78	0.004979\\
79	0.004304\\
80	0.004634\\
81	0.004628\\
82	0.004423\\
83	0.005836\\
84	0.003987\\
85	0.003903\\
86	0.003877\\
87	0.004036\\
88	0.003693\\
89	0.003648\\
90	0.004653\\
91	0.003688\\
92	0.004036\\
93	0.003647\\
94	0.004008\\
95	0.003961\\
96	0.004065\\
97	0.004846\\
98	0.004326\\
99	0.002836\\
100	0.004297\\
101	0.004626\\
102	0.005047\\
103	0.004023\\
104	0.004101\\
105	0.004529\\
106	0.004176\\
107	0.003187\\
108	0.003942\\
109	0.004135\\
110	0.00413\\
111	0.00445\\
112	0.004873\\
113	0.003634\\
114	0.003744\\
115	0.003431\\
116	0.003418\\
117	0.003454\\
118	0.003522\\
119	0.003449\\
120	0.003503\\
121	0.003057\\
122	0.003081\\
123	0.003156\\
124	0.003249\\
125	0.003148\\
126	0.003063\\
127	0.003147\\
128	0.003168\\
129	0.002885\\
130	0.003532\\
131	0.002771\\
132	0.002728\\
133	0.003232\\
134	0.003216\\
135	0.002686\\
136	0.00214\\
137	0.002067\\
138	0.002286\\
139	0.003111\\
140	0.00318\\
141	0.003196\\
142	0.002055\\
143	0.002785\\
144	0.002353\\
145	0.002194\\
146	0.003727\\
147	0.0029\\
148	0.002455\\
149	0.002477\\
150	0.002459\\
};

==> img/online_calib_plot_data/translation_error_data.tex <==
\addplot [color=mycolor1, line width=1pt]
  table[row sep=crcr]{%
1	9.65060022918023\\
2	3.72241601649895\\
3	3.42060257376163\\
4	2.11443393205203\\
5	2.80548739649831\\
6	2.99813719479121\\
7	1.66526240128351\\
8	1.35224344725879\\
9	1.34053449908488\\
10	1.24245108377934\\
11	1.38814137081094\\
12	0.850192848864273\\
13	0.624157641948158\\
14	0.677178348032737\\
15	0.680773942437944\\
16	0.808727623186806\\
17	0.638344944223968\\
18	0.694412056237932\\
19	0.802848285799145\\
20	0.899165252551257\\
21	0.858374716482661\\
22	0.87522687042183\\
23	1.0226291402389\\
24	1.00721876384459\\
25	1.19536257716936\\
26	1.34601088217705\\
27	1.2566098414632\\
28	1.26039869904071\\
29	1.30681388477804\\
30	1.31173062226517\\
31	1.25316293469477\\
32	1.08329315703593\\
33	0.996376321704113\\
34	0.988776979781131\\
35	0.9702123441231\\
36	0.969020197100758\\
37	1.05323021146136\\
38	1.01625147952972\\
39	1.0690479043736\\
40	1.06026666863489\\
41	1.04412571037125\\
42	1.10880718635635\\
43	0.990067190890207\\
44	1.18691927239683\\
45	1.17755664704581\\
46	1.19460221828056\\
47	1.17703053817567\\
48	1.1687680379567\\
49	1.21738214440074\\
50	1.24474013360416\\
51	1.35784585417158\\
52	1.31814471915281\\
53	1.16943210400153\\
54	1.08434024033136\\
55	1.03966721598566\\
56	1.02128933474181\\
57	1.02131817293567\\
58	1.05182432848709\\
59	1.0546425623797\\
60	1.06620053686461\\
61	0.94817228735794\\
62	0.903453371121143\\
63	0.961475981936543\\
64	0.92247862342028\\
65	0.921992475444742\\
66	0.918985123997567\\
67	0.918191976404945\\
68	1.08334412475502\\
69	1.1353849315289\\
70	1.12423880169625\\
71	1.21583755640889\\
72	1.27187401133489\\
73	1.13434590671068\\
74	1.1535899406691\\
75	1.11728306568482\\
76	1.11425282098852\\
77	1.18331029914945\\
78	1.19651597682411\\
79	1.20441447208963\\
80	1.20687122510503\\
81	1.21407230441037\\
82	1.33935835084234\\
83	1.33292732889752\\
84	1.40015538600851\\
85	1.36976669929959\\
86	1.39167870536198\\
87	1.41465865036012\\
88	1.48029845305669\\
89	1.49826447438275\\
90	1.47686509078207\\
91	1.60768500811342\\
92	1.65022931012225\\
93	1.68932494129302\\
94	1.66640013276161\\
95	1.74897777245241\\
96	1.64696560621466\\
97	1.79966917390366\\
98	1.66301060921376\\
99	1.72963940405741\\
100	1.68437155223748\\
101	1.64846535672946\\
102	1.62073432653626\\
103	1.58690780445298\\
104	1.57122995422126\\
105	1.55477395638038\\
106	1.5101449589555\\
107	1.51368857823211\\
108	1.50050905190833\\
109	1.48739304997862\\
110	1.38581186387087\\
111	1.2067369700006\\
112	1.09353867578202\\
113	0.598763980538592\\
114	0.459573428670086\\
115	0.26827488409098\\
116	0.119469780307646\\
117	0.0841954782370119\\
118	0.104070214669116\\
119	0.0407757286375674\\
120	0.218450674319555\\
121	0.12093995341565\\
122	0.223179680601403\\
123	0.124445353050719\\
124	0.0947462496962809\\
125	0.0332244240006965\\
126	0.0576949291734778\\
127	0.072721077162055\\
128	0.138854498081071\\
129	0.0763935780454016\\
130	0.163414932046422\\
131	0.111324019457091\\
132	0.136430500806401\\
133	0.108864539889222\\
134	0.113123143407479\\
135	0.125692043382079\\
136	0.118318857291921\\
137	0.108447920419136\\
138	0.122747383079886\\
139	0.107270104278851\\
140	0.112653572708316\\
141	0.109069488198031\\
142	0.119348898443134\\
143	0.120678663282562\\
144	0.123032121641987\\
145	0.126032434993286\\
146	0.106026427641371\\
147	0.111834079191862\\
148	0.105844089880934\\
149	0.111829157007432\\
150	0.110893427637855\\
};

  

==> img/online_calib_plot_data/verification_data.tex <==
\addplot [color=mycolor1, forget plot, line width=1pt]
    table[row sep=crcr]{%
1	4.16461284162957e-10\\
2	2.48766883503723e-08\\
3	5.76865314866019e-11\\
4	3.03246258670248e-11\\
5	1.45441813041887e-10\\
6	1.37523043716002e-12\\
7	8.73470125283886e-13\\
8	1.53428615976394e-12\\
9	6.46877173499325e-13\\
10	7.00631566652454e-13\\
11	2.80527166075523e-09\\
12	3.93871462498635e-09\\
13	4.45949033576711e-15\\
14	2.44415204226284e-09\\
15	5.59753240218843e-09\\
16	3.06264416293487e-11\\
17	4.3790684046137e-11\\
18	2.34309665492321e-12\\
19	7.81418987447944e-11\\
20	9.71004093103245e-14\\
21	9.28019148279265e-12\\
22	2.46611805860974e-10\\
23	2.09145352295451e-10\\
24	4.37307800964743e-11\\
25	1.2269265464715e-15\\
26	1.6479939074712e-12\\
27	2.71397379822004e-09\\
28	8.87183596593699e-09\\
29	1.54656579688422e-15\\
30	1.31549863594908e-18\\
31	1.31627438296956e-09\\
32	9.16828462108055e-18\\
33	5.82761953172087e-16\\
34	4.48426018540005e-16\\
35	8.95798812112452e-16\\
36	9.46725337014342e-16\\
37	1.62361958414197e-09\\
38	2.23898020007259e-15\\
39	4.95131969167717e-13\\
40	1.43410673961175e-15\\
41	1.96189820825457e-15\\
42	1.62291641765611e-15\\
43	5.36049725280042e-16\\
44	4.30654959294629e-16\\
45	2.35061777141708e-15\\
46	9.52878225071488e-11\\
47	5.26201843622887e-12\\
48	7.55959964765518e-17\\
49	3.38005558916093e-17\\
50	4.95523760912775e-17\\
51	6.45915063784171e-10\\
52	4.97498676870041e-16\\
53	3.7901907765354e-15\\
54	3.45265386497089e-15\\
55	1.55918523042137e-15\\
56	2.98408836083801e-15\\
57	5.62582996757356e-16\\
58	1.71079625561851e-16\\
59	4.01902536527544e-12\\
60	5.76477523125026e-16\\
61	1.03898560975103e-16\\
62	1.10385699153246e-10\\
63	1.73859218468117e-15\\
64	3.91077776052177e-10\\
65	3.88471306404898e-16\\
66	1.980607386852e-16\\
67	1.38739040985399e-16\\
68	1.00485132877924e-15\\
69	9.47656178896379e-10\\
70	4.3757174307546e-10\\
71	2.60390545197874e-15\\
72	2.48161830591127e-18\\
73	3.79785624562484e-16\\
74	6.22976707757887e-17\\
75	4.20951977708287e-10\\
76	6.1126177219288e-17\\
77	7.60687508653986e-17\\
78	3.11027023224816e-17\\
79	8.21337012510731e-10\\
80	1.11530793281411e-15\\
81	3.72626098358542e-15\\
82	1.67041177637962e-16\\
83	1.66048301907224e-11\\
84	2.68469109377363e-18\\
85	4.40011650481477e-13\\
86	1.04635855454977e-12\\
87	4.70393200763955e-15\\
88	2.57448734048376e-17\\
89	3.17386279983957e-10\\
90	4.03714330484325e-13\\
91	2.11304629471487e-10\\
92	3.15018240961406e-15\\
93	3.05417653533349e-15\\
94	3.95647794963613e-14\\
95	1.28040852774204e-15\\
96	9.05995475401304e-16\\
97	4.31177144389699e-17\\
98	3.11471370237632e-16\\
99	2.15121818065274e-09\\
100	9.77164793872221e-11\\
101	7.6805252305274e-11\\
102	1.10594563871781e-11\\
103	1.54904069614531e-15\\
104	4.52629386962564e-16\\
105	1.42364931629161e-09\\
106	3.16505207786712e-17\\
107	2.625947668034e-11\\
108	2.11035535754341e-15\\
109	1.36549792879642e-17\\
110	1.63663274851703e-16\\
111	8.08896243280581e-14\\
112	7.86270447312007e-13\\
113	2.93797106235276e-12\\
114	1.79859255534907e-12\\
115	8.54615291577965e-16\\
116	2.02528965820292e-16\\
117	2.80965896322739e-17\\
118	1.3083931301859e-18\\
119	1.34696175781729e-16\\
120	6.23054848455003e-18\\
121	1.7590956239864e-17\\
122	1.6309244483159e-17\\
123	1.54714768548501e-17\\
124	6.29536745314164e-19\\
125	1.60566004936413e-17\\
126	6.23674392553566e-18\\
127	5.97399153330504e-15\\
128	2.25514051876985e-17\\
129	1.31410741448181e-10\\
130	2.36537687140151e-12\\
131	5.62686294928824e-14\\
132	4.92030658640694e-17\\
133	4.48085485865369e-10\\
134	1.2068259909749e-11\\
135	4.22934491350993e-10\\
136	1.58797292487648e-11\\
137	3.06611660546521e-10\\
138	1.76577811890706e-10\\
139	5.33832730218916e-12\\
140	1.71899654728889e-12\\
141	1.18466951157307e-10\\
142	2.01008502707484e-10\\
143	4.19834621613223e-15\\
144	1.70243920957075e-11\\
145	3.69471201956827e-11\\
146	4.28358642316564e-12\\
147	8.70622711301401e-13\\
148	1.78534346301705e-10\\
149	2.30440846424448e-10\\
150	6.88250065966622e-11\\
};
